Towards Parallel Computing on the Internet: Applications, Architectures, Models and Programming Tools

The development of Internet wide resources for general purpose parallel computing poses the challenging task of matching computation and communication complexity. A number of parallel computing models exist that address this for traditional parallel architectures, and there are a number of emerging models that attempt to do this for large scale Internet-based systems like computational grids. In this survey we cover the three fundamental aspects -- application, architecture and model, and we show how they have been developed over the last decade. We also cover programming tools that are currently being used for parallel programming in computational grids. The trend in conventional computational models are to put emphasis on efficient communication between participating nodes by adapting different types of communication to network conditions. Effects of dynamism and uncertainties that arise in large scale systems are evidently important to understand and yet there is currently little work that addresses this from a parallel computing perspective.

==> Types_of_Parallel_Computation.tex <==
\section{Parallel Computing Techniques}

\subsection{Embarrassingly Parallel Computations}
Embarrassingly parallel computing is another technique used to
solve some large scale scientific computations. This is an ideal
parallel computation, with completely independent subtasks that
can be executed simultaneously with no communication between them.
Not much effort is required in terms of algorithm design and
techniques to parallelize problems of this type. These problems
can also be implemented efficiently. There are quite a number of
application that can be solved using this technique such as in
image processing, Monte Carlo simulation, DNA sequencing and
analysis of gene expression.
\subsection{Synchronous Computation}
\subsection{Grid Work-flow}


==> UMH.tex <==
\subsubsection{Uniform Memory Hierarchy (UMH)} The UMH model
captures the performance relevant aspect of hierarchical nature of
computer memory. It is used to model the higher performance of
algorithms achieved by tuned implementations that use data
movement strategies. Cost of moving data throughout the memory is
taken into consideration.

